Comparison between safety methods control barrier function vs. reachability analysis

This report aims to compare two safety methods: control barrier function and Hamilton-Jacobi reachability analysis. We will consider the difference with a focus on the following aspects: generality of system dynamics, difficulty of construction and computation cost. A standard Dubins car model will be evaluated numerically to make the comparison more concrete.

==> tex/Approach.tex <==
\section{Technical Approach}
\label{sec:technical_approach}
In this section, we propose a novel state-dependent directional metric (SDDM) and show that closed-loop trajectories of~\eqref{eq:lin_system} can be bounded in the SDDM by solving a convex optimization problem. We develop a feedback control law that exploits the trajectory bounds to stabilize the robot and follow the path $\Br$ adaptively, slowing down when safety may be endangered and speeding up otherwise.

\subsection{State-Dependent Directional Metric}
\label{sec:directional_sense}
As mentioned in the introduction, measuring safety using a static Euclidean norm may lead to system performance suffering from the \emph{corridor effect}. We propose a quadratic distance measure $\norm{\cdot}_\BQ$ that assigns priority to obstacles depending on the robot's moving direction. The level sets of $\norm{\cdot}_\BQ$ are ellipsoids $\C{E}_\BQ(\Bzero, \eta)$ whose shape and orientation are determined by the matrix $\BQ$. Our idea is to encode a desired directional preference in the distance metric via an appropriate choice of $\BQ$. Consider the example in Fig.~\ref{fig:norm_comparison}. A quadratic norm, well-aligned with the local environment geometry, may provide a more accurate evaluation of safety than a static Euclidean norm. Based on this observation, we propose a general construction of a directional matrix $\BQ[\Bv]$, in the direction of vector $\Bv$, that defines a state-dependent directional metric.
\begin{definition}%[Directional matrix]
	\label{def:directional_matrix}
	A \emph{directional matrix} associated with vector $\Bv$ and scalars $c_2 > c_1 > 0$ is defined as
	\begin{equation} \label{eq:directional_matrix}
	\BQ \brl{\Bv} =\begin{cases}
	c_2 \BI + (c_1 - c_2) \frac{\Bv \Bv^T}{\norm{\Bv}^2}, & \text{if}\ \Bv \neq 0, \\
	c_1 \BI, & \text{otherwise}.
	\end{cases}
	\end{equation} 
\end{definition}
The unit ellipsoid $\CE_{\BQ\brl{\Bv}}(\Bx, 1)$ centered at $\Bx$ generated by a directional matrix $\BQ\brl{\Bv}$ is elongated in the direction of $\Bv$.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\linewidth,valign=t]{fig/norm_comparison_Qdist.pdf}
	\includegraphics[width=0.48\linewidth,valign=t]{fig/norm_comparison_Edist.pdf}
	\caption{Robot (black dot) moving in direction $\Bv := \brl{\sqrt{2}/2, \sqrt{2}/2}$ (green arrow) along a corridor. The distances, measured by a quadratic norm $\norm{\cdot}_\BQ$ (left) and Euclidean norm $\norm{\cdot}$ (right), from the robot to the closest point (small blue square) on the wall (red line) are 1.41 and 0.71. The matrix $\BQ = [[2.5 -1.5],[-1.5, 2]]$ is defined as a \emph{directional matrix} $\BQ\brl{\Bv}$.}
	\label{fig:norm_comparison}
	%\vspace{-0.15in}
\end{figure}

\begin{lemma}
\label{lem:directional_metric}
For any vector $\Bv$, the directional matrix $\BQ \brl{\Bv}$ is symmetric positive definite.
\end{lemma}
\begin{proof}
Since $\Bv \Bv^T$ is symmetric, $\BQ\brl{\Bv}^T = \BQ\brl{\Bv}$. If $\Bv=\Bzero$, $\BQ\brl{\Bv} = c_1 \BI$ is positive definite. If $\Bv \neq \Bzero$ and $\Bq$ is arbitrary:
\begin{align*}
\Bq^T \BQ\brl{\Bv} \Bq  &= c_2 \Bq^T \Bq + (c_1 - c_2) \frac{(\Bq^T \Bv)^2}{\norm{\Bv}^2} \\
            &\geq c_2 \Bq^T \Bq + (c_1 - c_2) \frac{\norm{\Bq}^2 \norm{\Bv}^2}{\norm{\Bv}^2} = c_1 \norm{\Bq}^2,
\end{align*}
which follows from $c_2 > c_1$ and the Cauchy-Schwarz inequality. The proof is completed by noting that $c_1 > 0$.
\end{proof}
\subsection{Trajectory Bounds using SDDM}
\label{sec:ellipsoid_est}
Using a directional matrix, one can define an SDDM to adaptively evaluate the risk of surrounding obstacles. We will show how to use an SDDM to obtain bounds on the closed-loop trajectory of the constrained state $\Bx(t)$ in~\eqref{eq:lin_system}. Assume the robot is stabilized by a feedback controller $\Bu = -\BK \Bs$. The closed-loop dynamics are:
\begin{equation}
	\label{eq:LTI_closed_loop}
	\dot{\Bs} 	= \bar{\BA} \Bs \qquad
	\Bz 		= \BC \Bs 
\end{equation}
where $\bar{\BA} := (\BA - \BB \BK)$ is Hurwitz. Any initial state $\Bs_0 \coloneqq \Bs(t_0)$ will converge exponentially to the equilibrium point at origin. An output $\Bz$ is introduced to consider the constrained state $\Bx$. We are interested in measuring the maximum deviation of $\Bx(t)$ for $t \geq 0$ from the origin using a directional measure determined by the orientation of initial state $\Bx_0 \coloneqq \Bx(t_0)$ with respect to $\mathbf{0}$. Define an SDDM using the directional matrix:
\begin{equation}
\label{eq:directional_matrix_by_IC}
	 \BQ	\coloneqq \BQ \brl{\Bzero -\Bx_0} \in \pdm
\end{equation}
and choose output $\Bz(t) =  \BQ^{\frac{1}{2}} \Bx(t)$ so that $\BC \coloneqq \BQ^{\frac{1}{2}} \BP$, where $\BP \coloneqq \brl{\BI, \Bzero}$ is the projection matrix from $\Bs$ to $\Bx$. Note that $\Bz(t)^T \Bz(t) = \Bx(t)^T \BQ \Bx(t) = \norm{\Bx(t)}^2_{\BQ}$. Thus, measuring the maximum deviation of $\Bx(t)$ in the SDDM is equivalent to finding the output peak along the robot trajectory.
\begin{equation}
\label{eq:eta_def}
\eta(t_0) \coloneqq \max_{t\geq t_0} \norm{\rp(t)}_{\BQ}^2 = \max_{t\geq t_0}  \|\Bz(t)\|^2 
\end{equation} 
%subject to constraints from the robot dynamics~\eqref{eq:LTI_closed_loop} and the initial condition $\Bs_0$. 
We outline two approaches to solve this problem.

\subsubsection{Exact solution} % Exact solution by finding critical points
\label{sec:traj_est_exact_bound}
The output peak $\eta(t_0)$ can be computed exactly by comparing the values of $\|\Bz(t)\|^2$ at the boundary point $t = t_0$ and all critical points $\crl{t > t_0 \mid \frac{d}{dt} \|\Bz(t)\|^2 = 0}$. Since the closed-loop system in~\eqref{eq:LTI_closed_loop} is linear time-invariant, $\Bs(t)$ can be obtained in closed form. Let $\bar{\BA} = \BV \BJ \BV^{-1}$ be the Jordan decomposition of $\bar{\BA}$, where $\BJ$ is block diagonal. The critical points satisfy:
%$0 = \frac{d}{dt} \Bz(t)^T\Bz(t) = 2\Bz(t)^T \dot{\Bz}(t)= 2\prl{\BP \BV e^{\BJ (t-t_0)} \BV^{-1} \Bs_0}^T \!\!\BQ \prl{\BP \BV \BJ e^{\BJ (t-t_0)} \BV^{-1} \Bs_0}$
\begin{align}
0 &= \frac{d}{dt} \Bz(t)^T\Bz(t) = 2\Bz(t)^T \dot{\Bz}(t) \label{eq:critical_points}\\
&= 2\prl{\BP \BV e^{\BJ (t-t_0)} \BV^{-1} \Bs_0}^T \!\!\BQ \prl{\BP \BV \BJ e^{\BJ (t-t_0)} \BV^{-1} \Bs_0}.\notag
\end{align}
In general, an exact solution may be hard to compute due to the complicated expression of $e^{\BJ t}$.
%---------------------------------------------------------
\subsubsection{Approximate solution} % Upper bound by optimization
\label{sec:traj_est_upper_bound}
When an exact solution to~\eqref{eq:eta_def} is hard to obtain, we may instead compute a tight upper bound on $\eta(t_0)$. Given a $\BU \in \mathbb{S}^{n_s}_{>0}$,
\begin{equation}
\label{eq:invariant_ellipsoid}
\CE_{inv}  \coloneqq \crl{\Bxi \in \mathbb{R}^{n_s} \mid \Bxi^T \BU \Bxi \leq 1} 
\end{equation} 
is an invariant ellipsoid for the robot dynamics~\eqref{eq:LTI_closed_loop}, i.e., $\Bs(t) \in \CE_{inv}$ for all $t \geq t_0$. Instead of finding the peak value of $\|\Bz(t)\|^2$ along the state trajectory, we can compute it over the invariant ellipsoid $\CE_{inv}$. Since $\CE_{inv}$ contains the system trajectory, we have for all $t \geq t_0$:
\begin{equation}
\label{eq:relax_relation}
\norm{\Bz(t)}^2 \leq \eta(t_0) \leq \max_{\Bxi \in \CE_{inv}} \Bxi^T \BC^T \BC \Bxi  
\end{equation}
Obtaining the upper bound above is equivalent to solving the following semi-definite program~\cite[Ch.6]{boyd_LMI_book}:
\begin{equation}
\begin{aligned} \label{eq:SDP_UB}
& \underset{\BU, \delta}{\text{minimize}} & &  \delta  \\
& \text{subject to}
& &  \bar{\BA}^T \BU + \BU\bar{\BA} \preceq \Bzero, \;\; \Bs_0^T \BU \Bs_0 \leq 1 \\
&  & & \begin{bmatrix}
\BU 	& \BC^T \\
\BC 	& \delta \BI
\end{bmatrix} \succeq \Bzero ,\quad\;\;   \BU \succ \Bzero. 
\end{aligned}
\end{equation}


\begin{lemma}
\label{lemma:traj_bound}
For any initial condition $\Bs_0$ and associated constant directional matrix $\BQ$ in \eqref{eq:directional_matrix_by_IC}, the trajectory $\rp(t)$ under system dynamics~\eqref{eq:LTI_closed_loop} admits a tight ellipsoid bound, $\rp(t) \in \CE_\BQ(\Bzero, \eta(t_0)) \subseteq \CE_\BQ(\Bzero, \delta(t_0))$, for all $t \geq t_0$, where $\eta(t_0)$ is the solution to~\eqref{eq:eta_def} and $\delta(t_0)$ is the solution to~\eqref{eq:SDP_UB}.
 %\TORM{Getting the tight ellipsoid can be efficiently computed online}
\end{lemma}
\begin{proof}
%	 \CE_\BQ(\Bzero, \delta)
By definition, $\Bx(t) \in \CE_\BQ(\Bzero, \eta(t_0))$ is equivalent to $d^2_\BQ \prl{\Bzero, \Bx(t)} \leq  \eta(t_0)$. Since $\delta(t_0) =  \max_{\Bxi \in \CE_{inv}}\Bxi^T \BC^T \BC \Bxi$, inequality~\eqref{eq:relax_relation} yields
$\delta(t_0) \geq  \eta(t_0) \geq \norm{\Bz(t)}^2 = \norm{\Bx(t)}_\BQ^2 = d^2_\BQ \prl{\Bzero, \Bx(t)}$. Hence, $\Bx(t)\!\in\! \CE_\BQ(\Bzero, \eta(t_0)) \!\subseteq\!\CE_\BQ(\Bzero, \delta(t_0))$.\qedhere
\end{proof}
Now, we know how to find an accurate outer approximation of the system trajectory in the SDDM defined by~\eqref{eq:directional_matrix_by_IC}. We are ready to develop a feedback controller that utilizes the trajectory bounds to quantify the safety of the system with respect to surrounding obstacles, while following the navigation path towards the goal.
%=============================================================================
\subsection{Structure of the Robot-Governor Controller}
\label{sec:rgs_intro}
The problem of collision checking is simple for first-order kinematic systems since they can stop instantaneously to avoid collisions. We introduce a \emph{reference governor}~\cite{garone2016_ERG, kolmanovsky2014ref_cmd_gov}, a virtual first-order system:
$\dgp = \Bu_\gp$ with state $\gp \in \Rn$ and control input $\Bu_\gp \in \Rn$, which will serve to simplify the conditions for maintaining stability and safety concurrently. Our proposed structure of a path-following control design is shown in Fig.~\ref{fig:structure_safe_tracking}. The reference governor behaves as a real-time reactive trajectory generator that continuously regulates a reference signal for the real robot dynamics depending on risk level evaluation using SDDM. More precisely, we choose the real system's control input $\Bu$ so that the robot tracks the governor state $\gp$, while $\gp$ is regulated via $\Bu_\gp$ to ensure collision avoidance and stability for the joint robot-governor system.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth,valign=t]{fig/structure_safe_tracking_ssf_ver2.pdf}
	\caption{Structure of the proposed controller. A virtual reference governor adaptively conveys global navigation information to a local feedback controller based on the prediction of robot position trajectory. A local safe zone $\LS(\hat{\Bs})$, depending only on the current system state $\hat{\Bs}$, is constructed from an SDDM trajectory bound. A time-varying local goal $\Pi_{\LS(\hat{\Bs})} \Br$ is obtained by projecting the navigation path $\Br$ onto the local safe zone $\LS(\hat{\Bs})$. The governor chases the local goal and continuously sends its updated state $\gp$ as a reference signal to guide the local controller.
	}
	\label{fig:structure_safe_tracking}
\end{figure}

In detail, let $\tilde{\Bs} \coloneqq \Bs - \BP^T\Bg$ be the system state with the first element changed from $\Bx$ to $(\Bx - \gp)$ to make $\prl{\gp,\mathbf{0}}$ an equilibrium point. Choose a local controller for~\eqref{eq:lin_system} that tracks the governor state $\gp$:
\begin{equation}
\label{eq:local_feedback_controller}
\Bu = - \BK\, \tilde{\Bs}.
\end{equation}
Consider the augmented \emph{robot-governor system} with state $\hat{\Bs} = \prl{\tilde{\Bs}, \gp} \in \mathbb{R}^{(n_s + n)}$, coupling the real states with the governor state:
\begin{equation}
\label{eq:rgs_sum}
\dot{\hat{\Bs}}  = 
\begin{bmatrix}
\dot{\tilde{\Bs}} \\ \dgp
\end{bmatrix} = 
\begin{bmatrix}
	\bar{\BA} \tilde{\Bs} \\ \Bu_\Bg
\end{bmatrix}.
\end{equation}
Before proposing the design of the governor controller $\Bu_\gp(t)$, we analyze the behavior of the robot-governor system in the case of static governor.
\begin{lemma}
\label{lem:lyap_E}
If the governor is static, i.e., $\Bu_\gp(t)\equiv 0$ so that $\gp(t) \equiv \gp_0$, then the robot-governor system in~\eqref{eq:rgs_sum} is globally exponentially stable with respect to the equilibrium $\prl{\gp_0, \Bzero, \gp_0}$.
\end{lemma}
\begin{proof}
The subsystem $\dot{\tilde{\Bs}} = \bar{\BA} \tilde{\Bs}$ has an equilibrium at $\prl{\gp_0, \Bzero}$, which is globally exponentially stable because $\bar{\BA}$ is Hurwitz, while $\gp(t) \equiv \gp_0$ by assumption.
\end{proof}

In addition to guaranteeing stability for a static governor, we can use the ellipsoidal trajectory bounds from Lemma~\ref{lemma:traj_bound} to ensure safety.

\begin{theorem}
\label{thm:safety_static_gov}
Let $(\Bx_0 - \gp_0, \By_0, \gp_0)$ be any initial state for the robot-governor system in~\eqref{eq:rgs_sum} with $\Bx_0, \gp_0 \in \CF$. Suppose that $\Bu_\gp(t)\equiv \Bzero$ so that $\gp(t) \equiv \gp_0$. Let $\BQ \coloneqq \BQ \brl{\gp_0 - \Bx_0} \in \pdm$ be a constant directional matrix and suppose that the following safety condition is satisfied:
\begin{equation}
\label{eq:safety_condition}
\delta(t_0) \leq d_{\BQ}^2(\gp_0, \CO),
\end{equation}
where $\delta(t_0)$ is an upper bound for $\|\rp(t)-\gp_0\|_{\BQ}^2$ obtained according to Lemma \ref{lemma:traj_bound}. Then, the robot-governor system is globally exponentially stable with respect to the equilibrium $(\gp_0, \Bzero, \gp_0)$ and, moreover, the robot trajectory is collision free, i.e., $\rp(t) \in \CF$, for all $t \geq t_0$.
\end{theorem}


\begin{proof}
Since $(\Bg_0,\Bzero)$ is an equilibrium for $\dot{\tilde{\Bs}} = \bar{\BA} \tilde{\Bs}$, by Lemma~\ref{lemma:traj_bound}, $\rp(t) \in \CE_\BQ \prl{\gp_0, \delta(t_0)}$ for all $t \geq t_0$. From the safety condition in~\eqref{eq:safety_condition}, $\rp(t) \in \CE_\BQ \prl{\gp_0, \delta(t_0)} \subseteq \CE_\BQ(\gp_0, d^2_{\BQ} (\gp_0, \CO)) \subseteq \CF$ for all $t\geq t_0$. Stability is ensured by Lemma~\ref{lem:lyap_E}.
\end{proof}
%=================================================================
\subsection{Local Projected Goal and Governor Control Policy}
\label{sec:rgs_lpg_ug}
We established that the robot-governor system is stable and safe as long as the governor is static and \eqref{eq:safety_condition} holds. Next, we consider how to move the governor without violating these properties. Based on~\eqref{eq:local_feedback_controller}, we know that the robot will attempt to track the governor state. The main idea is to choose a time varying directional matrix $\BQ(t)  = \BQ \brl{\gp(t) - \rp(t)}$ to measure the system's safety. Since $\BQ(t)$ is positive definite (by Lemma~\ref{lem:directional_metric}), it can still be used to define an SDDM $\|\cdot\|_{\BQ(t)}$. Then, Lemma~\ref{lemma:traj_bound}, can still provide an accurate robot trajectory bound $\CE_{\BQ(t)} \prl{\gp(t), \delta(t)}$, which takes the robot's direction of motion into account. We need to design the governor control policy $\Bu_\gp(t)$ so that $\delta(t)$ never violates a time-varying version of the safety condition in~\eqref{eq:safety_condition}.

Our approach is to define an ellipsoid $\LS(\hat{\Bs})$, called a \emph{local safe zone}, centered at the governor state $\gp$, and have the size of $\LS(\hat{\Bs})$ determine how fast the governor can move. In the worst case, if system safety or stability are endangered, $\LS(\hat{\Bs})$ should shrink to a point, forcing the governor to remain static. Once there is enough leeway in the safety conditions in~\eqref{eq:safety_condition}, $\LS(\hat{\Bs})$ can grow, allowing the governor to move without endangering the safety or stability. 

\begin{definition}
\label{def:LS}
A \emph{local safe zone} is a time-varying set that at time $t$ depends on the robot-governor state $\hat{\Bs}(t)$ as follows:
\begin{equation}
\label{eq:LS}
\LS(\hat{\Bs}) \coloneqq \crl{ \Bq \in \CF \mid d_{\BQ}^2(\Bq, \gp) \leq  \max \prl{0, \DeltaE(\hat{\Bs})} },
\end{equation}
where $\BQ(t) \coloneqq \BQ \brl{\gp(t)-\rp(t)}$ is a directional matrix, determined by $\hat{\Bs}(t)$, and $\DeltaE(\hat{\Bs}(t)) \coloneqq d_{\BQ(t)}^2(\gp(t), \mathcal{O}) - \delta(t)$ is a measure of leeway to safety violation, determined by an upper bound $\delta(t)$ on $\|\Bx(\tau)-\Bg(\tau)\|_{\BQ(t)}$ for all $\tau \geq t$ and the directional distance $d_{\BQ(t)}^2(\gp(t), \mathcal{O})$ from the governor to the nearest obstacle.
\end{definition}
The term $\DeltaE(\hat{\Bs})$ estimates safety of the system based on local environment geometry and robot activeness. The requirement $\DeltaE(\hat{\Bs}) \geq 0$ only places a constraint on the magnitude $\norm{\dgp}$, so $\dot{\gp}/ \norm{\dgp}$ is a degree of freedom that can be utilized to make $\gp$ asymptotically tend to a desired goal. We define a local goal for the governor.

\begin{definition}%[Local projected goal]
\label{def:LPG}
A \emph{local projected goal} is the farthest point along the path $\Br$ contained in the local safe zone $\LS(\hat{\Bs})$:
\begin{equation}
\label{eq:local_projected_goal}
\alpha^* \coloneqq \max_{\alpha \in [0,1]} \crl{ \alpha \mid  \Br(\alpha) \in \LS(\hat{\Bs})} \quad \lpg(\hat{\Bs}) = \Br(\alpha^*)
\end{equation}
\end{definition}
The informal notation $\lpg(\hat{\Bs}) = \Pi_{\LS(\hat{\Bs})} \Br$ will be used for the local projected goal to emphasize that $\lpg(\hat{\Bs})$ is determined by projecting the path $\Br$ onto the local safe zone $\LS(\hat{\Bs})$. 
The structure of the complete closed-loop control policy is illustrated in Fig.~\ref{fig:structure_safe_tracking}, while the definitions of a local safe zone and a local projected goal are visualized in Fig.~\ref{fig:corridor_snapshot}.
We are finally ready to define the \emph{governor control policy}:
\begin{equation}
\label{eq:move2proj_goal}
\Bu_\gp \coloneqq -k_g \prl{ \gp - \lpg(\hat{\Bs}) } 
\end{equation}
where $k_g > 0$ is a control gain for the governor controller. We prove that the closed-loop system
is stable, safe, and asymptotically reaches the goal specified by the path $\Br$. We also informally claim that the path-following controller is fast due to the use of directional information for safety verification. This claim is supported empirically in Sec.~\ref{sec:evaluation}.

\begin{theorem}
\label{thm:safe_following}
Given a path $\Br$, the closed-loop robot-governor system~\eqref{eq:rgs_sum} with move-to-projected-goal~\eqref{eq:move2proj_goal} is asymptotically steered from any safe initial state $\hat{\Bs}_0$, i.e., $\DeltaE(\hat{\Bs}_0) > 0$ and $\Br(\alpha) \in \LS(\hat{\Bs}_0)$ for some $\alpha \in [0,1]$, to the goal state $\hat{\Bs}^* = (\Br(1), \Bzero, \Br(1))$ and the robot trajectory is collision-free for all time, i.e., $\rp(t) \in \CF$ for all $t \geq 0$.
\end{theorem}
\begin{proof}
From Thm.~\ref{thm:safety_static_gov}, we know that the robot-governor system~\eqref{eq:rgs_sum} will asymptotically converge to the equilibrium point $(\gp, 0, \gp)$ without collisions if the governor is static. The governor control policy in~\eqref{eq:move2proj_goal} allows the governor to move only when the interior of $\LS(\hat{\Bs})$ is nonempty. From Def.~\ref{def:LS}, this happens only if the safety condition is strictly satisfied, i.e., $\DeltaE(\hat{\Bs}) = d_{\BQ(t)}^2(\gp(t), \mathcal{O}) -  \delta(t) > 0$. Since $\rp$ approaches $\gp$, $\DeltaE(\hat{\Bs})$ eventually becomes strictly positive and the set $\LS(\hat{\Bs})$ becomes an ellipsoid in free space with non-empty interior. Since initially $\Br(\alpha) \in \LS(\hat{\Bs}_0)$ for some $\alpha \in [0,1]$, the local projected goal in~\eqref{eq:local_projected_goal} will be well defined and when $\LS(\hat{\Bs})$ grows, the projected goal will move further along the path $\Br$, i.e., the path length parameter $\alpha$ will increase. Since the system dynamics are continuous, $\DeltaE(\hat{\Bs})$ cannot suddenly become negative without crossing zero.  If $\DeltaE(\hat{\Bs}) \downarrow 0$, the local energy zone $\LS(\hat{\Bs})$ shrinks to a point, i.e., $\LS(\hat{\Bs}) = \crl{\gp}$, and hence the governor stops moving and waits until the robot catches up. When the governor is static, and since the safety condition in~\eqref{eq:safety_condition} is satisfied, Thm.~\ref{thm:safety_static_gov} again guarantees that the robot can approach the governor without collisions, increasing $\DeltaE(\hat{\Bs})$ in the process. Once $\DeltaE(\hat{\Bs})$ goes above $0$, the governor starts moving towards the goal again by chasing the projected goal. Note that the local projected goal always lies on the navigation path inside the free space, i.e., $\lpg \in \Br \subset \mathring{\CF}$, so the robot-governor system cannot remain stuck at any configuration except $\hat{\Bs}^* = (\Br(1), \Bzero, \Br(1))$. Using LaSalle's Invariance Principle~\cite{khalil2002nonlinear}, we can conclude that the largest invariant set is the point where both the robot and the governor are stationary at the goal location $\Br(1)$.
\end{proof}


==> tex/Evaluation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\linewidth]{fig/demo_opt_traj_ellipse2D_vSG1C7E0M0}%
\hfill %
\includegraphics[width=0.22\textwidth]{fig/demo_opt_traj_ellipse2D_vSG1C7E2M0}%
\caption{Trajectory bounds comparison between a Euclidean metric (left) and an SDDM (right). The governor is fixed at the origin while the robot's initial conditions are $\rp_0 = (-2, 0)$ and $\rv_0 = (0, 2)$. The change of the trajectory bounds over time is illustrated via ellipsoids with different colors, starting from cold/blue and converging towards warm/red.}
\label{fig:traj_est_comp}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth,valign=t]{fig/corridor_snapshot.pdf}
	\caption{Comparison of controller 1 (top) and 2 (bottom) in a corridor simulation. A snapshot is shown at the same time instant for both controllers. The local energy zone (yellow) resulting from the proposed SDDM trajectory bounds fits the corridor environment well, leading to fast, yet safe, movement.\label{fig:corridor_snapshot}}%
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.24\linewidth]{fig/sparse_ball173.pdf}%
	\hfill%
	\includegraphics[width=0.24\linewidth]{fig/sparse_ellipse110.pdf}
	\hfill%
	\includegraphics[width=0.24\linewidth]{fig/rgs_traj_ball.pdf}%
	\hfill%
	\includegraphics[width=0.24\linewidth]{fig/rgs_traj_ellipse.pdf}
	\caption{Simulation of the robot-governor system tracking a piecewise-linear path (black) in an environment with circular obstacles (dark gray circles). The start and end of the path are indicated by a red and green star, respectively. The two plots on the left show that the robot at around the same location behaves differently due to different distance measures. The controller using Euclidean distance is overly cautious with respect to lateral obstacles resulting in conservative motion. The system employing SDDM trajectory bounds has a larger local safe zone, which helps the robot turn fast and smoothly. The two plots on the right show the trajectories followed by the systems employing the two controllers. The velocity profiles are shown as magenta arrows perpendicular to the robot path. The controller based on SDDM trajectory bounds (rightmost) results in higher velocities compared to the controller using Euclidean ball invariant sets. Note that the path followed by the robot (green line) is also smoother, especially when turning, for the directional controller despite the higher velocity.}
	\label{fig:static_sparse_sim}
\end{figure*}

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth,valign=t]{fig/Eta_max_comparison.pdf}
	\vspace{-2ex}
	\caption{Output peak $\norm{\rp(t)}^2_{\BQ(t)}$ from the trajectory followed in Fig.~\ref{fig:static_sparse_sim}. The red curve is $\eta(t, \BQ(t))$ obtained analytically from eq.~\eqref{eq:critical_points}. The blue curve is $\delta(t)$ computed from the SDP optimization in eq.~\eqref{eq:SDP_UB}.  It is clear that $\delta(t)$ is an upper bound for $\eta(t, \BQ(t))$, and the bound is tight at certain moments. Analytical bounds are used in simulation, while optimization bounds are computed for comparison purpose. }
	\label{fig:Eta_max_comparison}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{fig/LMOG_10600.png}%
	\caption{Snapshot of the robot-governor system navigating the environment shown in Fig.~\ref{fig:complex_cooridor_sim}. Streaming lidar scan measurements (red dots) are used to update an occupancy grid map (black lines and white regions in top plot) of the unknown environment. An acceleration-controlled robot (green dot) follows a virtual governor (blue dot) whose motion is modulated based on the local energy zone (yellow ellipse) and the directional distance to obstacles (gray ellipse). A navigation path (blue line) is periodically replanned using an $A^*$ planner and an inflated occupancy grid map (bottom plot).}
	\label{fig:complex_cooridor_sim_2D_status}
\end{figure}

\section{Evaluation}
\label{sec:evaluation}
Consider an acceleration-controlled robot, stabilized by a proportional-derivative (PD) controller:
\begin{equation}
\label{eq:double_integrator}
\ddrp = \Bu \coloneqq -2 k \rp - \zeta \drp.
\end{equation}
The closed-loop robot-governor system is:
\begin{equation}
\label{eq:closed-loop_rgs_double_integrator}
\dot{\hat{\Bs}}  = 
\begin{bmatrix}
\drp \\
\ddrp\\
\dgp
\end{bmatrix} = 
\begin{bmatrix}
	\rv \\
	- 2 k (\rp - \gp) - \damping \rv \\
	-k_g (\gp - \lpg(\hat{\Bs}))
\end{bmatrix}
\end{equation}
Several experiments will be shown to compare the performance of two path-following controllers:
\begin{itemize}
    \item \textbf{Controller~1}~\cite{Gov_ICRA17}: uses a Lyapunov function to ensure stability and collision avoidance. The robot's kinetic and potential energy, i.e., $E(\hat{\Bs}) \coloneqq k \norm{\rp - \gp}^2 + \frac{1}{2} \norm{\rv}^2$ is used to define a spherical local safe zone.
    \item \textbf{Controller~2} (ours): uses SDDM trajectory bounds (Lemma~\ref{lemma:traj_bound}) to define an ellipsoidal local safe zone. %  (Def.~\ref{def:LS})
\end{itemize}
In visualizations, the governor and robot positions are shown by a blue and green dot, respectively. A light-gray ellipse/ball indicates the distance from the governor to the nearest obstacles, while the local safe zone $\LS(\hat{\Bs})$ is indicated by a yellow ellipse/ball. The projected goal $\lpg$ is shown as a small red dot at the boundary of $\LS(\hat{\Bs})$. The controller parameters were $k = k_g = 1$, $\damping = 2 \sqrt{2}$, $c_1 = 1, c_2 = 4$.

\textbf{Trajectory Prediction using Different Metrics.\;} First, we demonstrate that predicting the robot trajectory using our directional metric has some desirable properties for enforcing safety constraints. Fig.~\ref{fig:traj_est_comp} compares trajectory bounds obtained from Lemma~\ref{lemma:traj_bound} for~\eqref{eq:double_integrator} using a Euclidean metric and an SDDM. Since the robot dynamics are simple, a tight directional trajectory bound $\CE_{\BQ_t}(\Bzero, \eta(t))$ can be obtained from an exact computation of the critical points according to~\eqref{eq:critical_points}. It is clear that the ellipsoid bounds on the system trajectory are less conservative (smaller area/volume) than the spherical bounds at beginning. 
%as long as the damping $\damping$ is relatively large compared to $\lambda_{\max}(\BQ)$.
Unlike a Lyapunov function, the ellipse $\CE_{\BQ(t)}(\Bzero, \eta(t))$ bounding the robot trajectory is not forward invariant. It can be shown that requiring invariance of directional ellipsoids ($\CE_{\BQ_{(t_1)}} \subset \CE_{\BQ_{(t_2)}} \,\, \forall t_2 \geq t_1$) would need infinite damping unless $\BQ = k \BI$ for some $k > 0$, causing the metric to lose directionality. In contrast to control designs based on Lyapunov function invariance, we make an interesting observation that a safe and stable controller can be defined even if the sets containing the system trajectory are not strictly shrinking over time.

\textbf{Corridor Environment.\;} We show that utilizing a directional metric in the control design alleviates the corridor effect discussed in Sec.~\ref{sec:introduction}. We setup a simulation requiring a robot to navigate through a corridor (Fig.~\ref{fig:corridor_snapshot}). The results show that controller 1, using a Lyapunov function with spherical level sets, suffers from the corridor effect while the proposed controller 2, making directional predictions about the system trajectory, does not.

\textbf{Sparse Environment with Circular Obstacles.\;} This experiment compares the two controllers in a longer path-following task in an environment with circular obstacles. Snapshots illustrating how the two controllers judge distances to obstacles and define a local energy zone are shown in Fig.~\ref{fig:static_sparse_sim}. It can be seen that the controller equipped with a directional sensing ability has a better understanding of the local environment geometry, leading to a larger, elongated local safe zone set. As a result, controller 2 does not need to slow down for low-risk lateral obstacles, leading to smoother and faster navigation. The directional bounds on the robot trajectory obtained analytically, according to eq.~\eqref{eq:critical_points}, and from the SDP in eq.~\eqref{eq:SDP_UB} are compared in Fig.~\ref{fig:Eta_max_comparison}.

\textbf{Unknown Environment with Arbitrary Obstacles.\;} This experiment demonstrates that our controller can work in a complex unknown environment, shown in Fig.~\ref{fig:complex_cooridor_sim}, relying only on local onboard measurements. The directional distance $d_{\BQ(t)}^2(\gp(t), \mathcal{O})$ from the governor to the obstacles is computed from the latest lidar scans. The path $\CP$ is re-planned from the current governor position to the goal using an occupancy grid map constructed from the lidar scans over time, as illustrated in Fig.~\ref{fig:complex_cooridor_sim_2D_status}. 


==> tex/Notations.tex <==
\section{Notation}
%For conciseness, let us first introduce our notations used in the rest of this paper.
Let $\pdm$ and $\psdm$ denote the set of $n\times n$ symmetric positive and semi-definite matrices. Let $\succ$ and $\succeq$ denote the generalized inequalities associated with $\pdm$ and $\psdm$. Denote the Euclidean ($\ell^2$) norm by $\norm{\Bx}$ and the quadratic norm induced by $\BQ \in \pdm$ as $\norm{\Bx}_\BQ \coloneqq \sqrt{ \Bx^T \BQ \Bx}$. Let $\lambda_{\max}(\BQ)$ and $\lambda_{\min}(\BQ)$ be the maximum and minimum eigenvalues of $\BQ$. Let $d_\BQ(\Bx, \C{A}) \coloneqq \inf_{\mathbf{a} \in \C{A}} \norm{\Bx-\mathbf{a}}_\BQ$ denote the quadratic norm distance from a point $\Bx$ to a set $\C{A}$. Given $\BQ \in \pdm$ and scaling $\eta \geq 0$, denote the associated ellipsoid centered at $\Bq \in \Rn$ by $\C{E}_\BQ(\Bq , \eta) \coloneqq \crl{\Bx \in \Rn \mid (\Bx-\Bq )^T \BQ (\Bx-\Bq ) \leq \eta}$.

